Lipschitz Continuity in Model-based Reinforcement Learning

We examine the impact of learning Lipschitz continuous models in the context of model-based reinforcement learning. We provide a novel bound on multi-step prediction error of Lipschitz models where we quantify the error using the Wasserstein metric. We go on to prove an error bound for the value-function estimate arising from Lipschitz models and show that the estimated value function is itself Lipschitz. We conclude with empirical results that show the benefits of controlling the Lipschitz constant of neural-network models.

==> finite.tex <==
ML's argument for why any finite MDP can be viewed as a Lipschitz model class.

T(s,a,s') is the transition function for the MDP.

Define an ordering on states s1,...,sn 
(for notational simplicity, define s0 to be a state that is unreachable, T(s,a,s0) = 0 for all s,a) and use it to define a cumulative transition probability function C(s,a,si) = sum_{j = 0 to i} T(s,a,sj). 

Because S and A are finite, there are at most a finite set of values in {C(s,a,si) | s in S, i in 0 to n, a in A}. Let k be the size of this set. Sort these values and define ci to be the ith smallest value (so c0 < ci < ck). Note that c0 = 0 (since no state can reach s0 so C(s,a,s0)=0) and ck = 1 (since the sum of the transition probabilities for any s,a is 1 so C(s,a,sn)=1).

For i=1 to k and j=1 to n, define Ti(s,a) = sj if
  C(s,a,s{j-1}) < ci <= C(s,a,sj)

Define:
gi = ci-c{i-1} for i from 1 to k,

The probability of transitioning to sj from s given action a is

sum_{i st Ti(s,a) = sj} gi
= sum_{i st C(s,a,s{j-1}) < ci <= C(s,a,sj)}  ci-c{i-1}
=  C(s,a,sj) - C(s,a,s{j-1})
= T(s,a,sj)

As for the Lipschitz condition, we can define distances to be d(si,sj) = |i-j| so K <= 9.

example

T:
0.2 0.2 0.0 0.0 0.6
0.0 0.3 0.3 0.2 0.2
0.0 0.4 0.0 0.0 0.6
0.1 0.1 0.0 0.3 0.5

C:
    s1  s2  s3  s4  s5
s1 0.2 0.4 0.4 0.4 1.0
s2 0.0 0.3 0.6 0.8 1.0
s3 0.0 0.4 0.4 0.4 1.0
s4 0.1 0.2 0.2 0.5 1.0

c1 0.0
c2 0.1
c3 0.2
c4 0.3
c5 0.4
c6 0.5
c7 0.6
c8 0.8
c9 1.0

T2 0.1 s1 s2 s2 s1
T3 0.1 s1 s2 s2 s2
T4 0.1 s2 s2 s2 s4
T5 0.1 s2 s3 s2 s4
T6 0.1 s5 s3 s5 s4
T7 0.1 s5 s3 s5 s5
T8 0.2 s5 s4 s5 s5
T9 0.2 s5 s5 s5 s5

T induced:
0.2 0.2 0.0 0.0 0.6
0.0 0.3 0.3 0.2 0.2
0.0 0.4 0.0 0.0 0.6
0.1 0.1 0.0 0.3 0.5




HOLD:


Because S and A are finite, there are at most a finite set of values in {C(s,a,s') | s,s' in S, a in A} U {0}. Let k be the size of this set. Sort these values and define ci to be the ith smallest value (so c1 < ci < ck). Note that c1 = 0 and ck = 1.

For i>1, define Ti(s,a) = s' if
 c{i-1} <  C(s,a,s')  <= ci

gi = ci-c{i-1}


The probability of transitioning to s' from s given action a is

sum_{i st Ti(s,a) = s'} gi
= 


